Deterministic Consistency: A Programming Model for Shared Memory Parallelism

The difficulty of developing reliable parallel software is generating interest in deterministic environments, where a given program and input can yield only one possible result. Languages or type systems can enforce determinism in new code, and runtime systems can impose synthetic schedules on legacy parallel code. To parallelize existing serial code, however, we would like a programming model that is naturally deterministic without language restrictions or artificial scheduling. We propose "deterministic consistency", a parallel programming model as easy to understand as the "parallel assignment" construct in sequential languages such as Perl and JavaScript, where concurrent threads always read their inputs before writing shared outputs. DC supports common data- and task-parallel synchronization abstractions such as fork/join and barriers, as well as non-hierarchical structures such as producer/consumer pipelines and futures. A preliminary prototype suggests that software-only implementations of DC can run applications written for popular parallel environments such as OpenMP with low (<10%) overhead for some applications.

==> arch.tex <==
\subsection{Architectural Variants}

Since architectures constantly evolve,
different processors added to a cloud at different times
may implement different architecture variants or optional features.
%such as vector processing extensions.
While a cloud vendor may define
the minimum feature set any its processors will have
(e.g., ``at least SSE2''~\cite{intel09}),
some processors are likely to have more features (e.g., SSE3).
Replay-based mechanisms often require {\em exact} correspondence, however.
If an application uses the x86's {\tt CPUID} instruction
to detect and take advantage of SSE3,
then the same code replayed on a processor without SSE3
will follow a different path at least at certain times,
breaking any state correspondence tests that occur during those times.

\com{
We generally expect a cloud computing provider
to standardize the set of processors used in a cluster to some degree,
or at least to allow the customer to choose
a particular processor class or model
having a particular minimum feature set,
such as supporting ``at least'' SSE2~\cite{intel09}.
When a computation needs to be replayed on or migrated to another machine
in a cluster,
however,
it is not sufficient to standardize only the {\em minimum} feature set:
an {\em exact} feature set must be specified and standardized
throughout the cluster.

Consider for example an application that is first run
on a machine that supports not only the cluster's minimum feature set of SSE2,
but also an additional optional architecture feature such as SSE3.
The application or a library it links with
may contain code that uses the {\tt CPUID} instruction
to detect the processor's support for SSE3
and reconfigure some code path to take advantage of SSE3 instructions.
Even if the alternate code path eventually computes
precisely the same arithmetic result,
the application's execution trace is still affected:
it will probably execute a different number of instructions
than the same application running on a processor without SSE3,
and the values of the processor registers (particularly EIP)
will be different at least at certain points during execution.
If the same application is then replayed on another processor without SSE3,
the replayed execution trace will diverge at those points,
potentially causing failures, false alarms
in fault tolerance or accountability mechanisms, etc.
Worse, if an application starts running on a processor with SSE3,
and then is dynamically migrated to a processor without SSE3
after the application's code path has been configured for the first processor,
then the application will take an illegal instruction exception
the first time it tries to execute an SSE3 instruction after migration.
}

Intel's VMX~\cite{intel09} and AMD's SVM~\cite{amd07} extensions
enable a VMM to intercept {\tt CPUID}
and ``lie'' about supported processor features.
This intercept is only available to a VMM
and not to OS- or application-level virtualizers,
however,
and incorrect or malicious code could still follow divergent code paths
on different processors
simply by trying to use extensions without testing for them.
For this reason,
fully standardizing behavior across current x86 processors
requires both falsifying {\tt CPUID} results
{\em and} trapping actual attempts to access ``hidden'' extensions.
Our \dvus prototype builds on the vx32~\cite{ford08vx32} sandbox,
which uses dynamic instruction rewriting to sandbox guest code;
we are leveraging this instruction rewriting capability
to restrict the visible architecture to an exact
set of features and instructions.
Static analysis techniques
like those used in PittSFIeld~\cite{mccamant06evaluating}
	% XXX or Google's NaCl~\cite{XXX}
may also be applicable.

\com{
from guest OSes and applications, for example,
and thereby standardize the architectural feature set available
across a virtualized cluster.
these extensions may be unavailable, however,
or a cloud computing {\em customer} may wish
wish to create at the guest OS level
a deterministic execution environment
with a standardized architectural feature set
across virtual machines provided by more than one cloud computing vendor
(e.g., for scaling beyond what one vendor can support
or for cross-vendor fault tolerance or accountability).
In this case,
instruction rewriting or other approaches may be required
to standardize the architectural feature set
by masking the appropriate CPUID feature flags
and disallowing the execution of corresponding extended instructions.
Since our vx32 virtualization platform
performs instruction rewriting anyway for sandboxing purposes,
we intend to leverage vx32's rewriting
to provide architecture standardization in our deterministic environment.
We do not expect this standardization to incur a significant performance cost
beyond the inherent cost of vx32's dynamic rewriting itself,
since architecture standardization only affects instructions
that are executed rarely (e.g., CPUID)
or should not be executed at all (the disabled extension instructions).
}

\subsection{Architecturally Unpredictable Results}

Most architectures
leave some results of some instructions unspecified.
The x86 for example
leaves undefined the effects of many instructions
on certain condition codes.
\com{	probably unnecessary
Similarly, architectures often leave results unspecified
in certain boundary conditions:
the x86 architecture leaves the arithmetic result of SHLD and SHRD instructions
undefined if the shift count is greater than the operand size,
since this situation is architecturally considered a programmer error.
}
Though normal applications
avoid depending on undefined results,
buggy or malicious code could diverge across processors
by using undefined results.
Even with correct code,
undefined values may persist in registers or condition codes for short periods,
breaking any cross-processor state correspondence tests
that might occur during those periods.
\com{
in the way processors 
processor implementation differences can affect the behavior
of buggy or malicious code.
Even if the application code is correct,
undefined results may persist in processor registers for short times.
If a Peer Review~\cite{XXX} system
checkpoints an application process
shortly after the execution of a DIV instruction, for example,
and a ``reviewer'' node replays the process up to that same point
to check the resulting state,
then any differences in the way the respective processors
leave the condition codes after the DIV instruction
result in a false alarm.
}

As with feature set standardization,
\dvus builds on vx32's instruction rewriting capability
to canonicalize undefined results across processors.
The performance cost of this canonicalization
may an issue because it involves a number of common unprivileged instructions.
Fortunately, the most common x86 instructions such as ADD and MOV
are already fully deterministic,
and most of the problematic instructions
require only a small and simple rewrite.
An $n$-bit x86 shift instruction, for example,
leaves the OF condition code undefined if $n \ne 1$,
but can be canonicalized by replacing it
with an $(n-1)$-bit shift followed by a $1$-bit shift.

\com{
%Compared with architectural variants as discussed above,
Canonicalizing unpredictable results present a greater challenge
to providing full determinism
because many common unprivileged instructions are involved.
Processor architectures could be modified to specify all results precisely,
but processor designers may be resistant to giving up
the implementation flexibility afforded by architecturally undefined results.
\com{
The ideal solution may be simply to modify the architecture
so that the results of all instructions
(or at least all unprivileged instructions)
are fully specified.
The practice of leaving semantically inapplicable or boundary-case results
undefined is common, however,
and processor architects may be resistant to giving up this practice
because of the flexibility it provides at processor implementation time.
}
A more practical solution for now is therefore

If we wish to provide fully deterministic execution
across a heterogeneous set of existing processors, therefore,
the options appear to be:
(a) use instruction rewriting techniques, as in vx32,
to rewrite instructions that produce architecturally undefined results
so that they always behave in a standard fashion for all inputs;
or
(b) use static code analysis techniques,
analogous to those used for sandboxing
in PittSField~\cite{XXX} and NaCl~\cite{XXX},
to verify that application code never depends on unpredictable results,
and to identify and mask any unpredictable values
that might otherwise appear in execution state snapshots.
The latter approach may be less costly in terms of performance,
but requires substantial changes to compiler toolchains
and potentially to application code,
whereas the former approach works on standard compiled
or hand-written application code.
We are currently exploring the former approach,
by developing extensions to vx32
to canonicalize the behavior of all instructions available to guests;
the static analysis approach is also promising however
and merits further study.

We do not yet have performance results on the cost
of instruction behavior canonicalization,
but we expect the cost to be small,
since the most common x86 instructions such as ADD and MOV
are already fully deterministic,
and most of the problematic instructions
can be canonicalized using a small and simple rewrite.
An $n$-bit x86 shift instruction, for example,
leaves the OF condition code undefined if $n \ne 1$,
but can be canonicalized by replacing it
with an $(n-1)$-bit shift followed by a $1$-bit shift.
}%com



==> bio-baf.tex <==
\newpage
\pagenumbering{arabic}
\renewcommand{\thepage} {F--\arabic{page}}
\begin{center}
{\Large{\bf PI Biography: Bryan A. Ford}}\\*[3mm]
\end{center}

\subsection*{Bryan A. Ford}

\com{
Bryan A. Ford is an Assistant Professor in Computer Science at Yale University.
Bryan Ford received a BSc in Computer Science from University of Utah in 1998,
a Masters in Computer Science from MIT in 2002,
and a PhD in Computer Science from MIT in 2008.
For the academic year of 2008 to 2009,
he is a post-doctoral research scientist
at the Max Planck Institute for Software Systems.
His research interests are eclectic,
drawing on techniques from operating systems, networking, virtualization,
storage systems, programming languages, and formal methods.
His current focus is on the creation of a new, fully decentralized
("peer-to-peer") paradigm for applications distributed across personal devices
and Internet services, built from novel OS abstractions such as personal groups,
structured streams, and lightweight sandboxing.
For details, see http://www.bford.info/.
}

\subsubsection*{(a) Professional Preparation}

\begin{center}
\begin{tabular}{llll}
University of Utah			& Computer Science	& BSc & 1998 \\
Massachusetts Institute of Technology	& Computer Science	& MSc & 2002 \\
Massachusetts Institute of Technology	& Computer Science	& PhD & 2008 \\
Max Planck Institute for Software Systems & Computer Science	& Postdoc
								& 2008--2009 \\
\end{tabular}
\end{center}

\subsubsection*{(b) Appointments}

% The guidelines say "all"; does it really mean "all"?
% should it include consultancies?

\begin{itemize}
\item	{\bf Yale University}, New Haven, CT, 2009--: \\
	{\em Assistant Professor of Computer Science}.

%\item	{\bf Nuvoiz, Inc.}, Mountain View, CA, 2006: \\
%	{\em Consultant} on NAT traversal technology for Voice-over-IP.

\item	{\bf Phobos, Inc.}, Salt Lake City, UT, 1998--2000: \\
	{\em Engineer},
	designing Internet traffic management devices
	in a startup acquired by SonicWALL, Inc.

\item	{\bf Sleepless Software}, Salt Lake City, UT, 1993--1998: \\
	{\em Co-founder} of a small company developing entertainment software
	for MS-DOS, Windows, and Java.

\item	{\bf University of Utah}, Salt Lake City, UT, 1992--1997: \\
	{\em Research Associate}, serving as architect 
	in several systems research projects; see publications.

\item	{\bf Open Software Foundation}, Cambridge, MA, 1993: \\
	{\em Consultant} on integrating fast RPC and migrating threads
	into OSF Mach kernel.

\item	{\bf Hewlett-Packard}, McMinnville, OR, 1992: \\
	{\em Software Engineer} developing cardiology database management tools.

%\item	{\bf Designing Minds}, Logan, UT, 1991--1992: \\
%	{\em Consultant} on device driver design
%	for high-speed data compression hardware.

\item	{\bf Waterford Institute}, Provo, UT, 1989--1991: \\
	{\em Software Engineer}, creating educational curricula and software
	with a team of teachers.

%\item	{\bf Designing Minds}, Logan, UT, 1987--1988: \\
%	{\em Consultant}, developing a painting program for bitmapped graphics
%	and animation on Amiga computers, published 1988.
\end{itemize}

\subsubsection*{(c) Publications}

\paragraph{Most Relevant:}
\begin{enumerate}
\item	{\it Vx32: Lightweight User-level Sandboxing on the x86},
	Bryan Ford and Russ Cox.
	USENIX Annual Technical Conference, June 2008.
	{\em Awarded Best Student Paper.}
	~ \url{http://bford.info/pub/os/vx32-abs.html}

\item	{\it VXA: A Virtual Architecture for Durable Compressed Archives},
	Bryan Ford.
	4th USENIX Conference on File and Storage Technologies,
	December 13-16, 2005.
	~ \url{http://bford.info/pub/os/vxa/}

\item	{\it Interface and Execution Models in the Fluke Kernel},
	Bryan Ford, Mike Hibler,
	Jay Lepreau, Roland McGrath, and Patrick Tullmann.
	USENIX Symposium on Operating Systems Design and Implementation (OSDI),
	February 1999.
	~ \url{http://www.bford.info/pub/os/atomic-osdi99.pdf}

\item	{\it The Flux OSKit: A Substrate for Kernel and Language Research},
	Bryan Ford, Godmar Back, Greg Benson, Jay Lepreau, Albert Lin,
	and Olin Shivers.
	16th ACM Symposium on Operating System Principles (SOSP), October 1997.
	~ \url{http://www.bford.info/pub/os/oskit-sosp16.pdf}

\item	{\it Microkernels Meet Recursive Virtual Machines},
	Bryan Ford, Mike Hibler, Jay Lepreau, Patrick Tullmann,
	Godmar Back, and Stephen Clawson.
	USENIX Symposium on Operating Systems Design and Implementation (OSDI),
	October 1996.
	~ \url{http://www.bford.info/pub/os/fluke-rvm.pdf}
\end{enumerate}

\paragraph{Other Publications:}
\begin{enumerate}
\item	{\it Efficient Cross-Layer Negotiation},
	Bryan Ford and Janardhan Iyengar.
	HotNets-VIII, October 22-23, 2009.
	~ \url{http://bford.info/pub/net/nego-abs.html}

\item	{\it Structured Streams: a New Transport Abstraction},
	Bryan Ford.
	ACM SIGCOMM, August 2007.
	\\ \url{http://www.bford.info/pub/net/sst-abs.html}

\item	{\it Persistent Personal Names for Globally Connected Mobile Devices},
	Bryan Ford, Jacob Strauss, Chris Lesniewski-Laas,
	Sean Rhea, Frans Kaashoek, and Robert Morris.
	7th USENIX Symposium on
		Operating Systems Design and Implementation (OSDI),
	November 2006.
	\\ \url{http://www.bford.info/pub/net/uia-osdi-abs.html}

\item	{\it Peer-to-Peer Communication Across Network Address Translators},
	Bryan Ford, Pyda Srisuresh, and Dan Kegel.
	USENIX Annual Technical Conference, April 2005.
	\\ \url{http://www.bford.info/pub/net/p2pnat-abs.html}

\item	{\it Parsing Expression Grammars:
	A Recognition-Based Syntactic Foundation},
	Bryan Ford.
	31st Symposium on Principles of Programming Languages (POPL),
	January 2004.
	\\ \url{http://www.bford.info/pub/lang/peg.pdf}

\end{enumerate}

\subsubsection*{(d) Synergistic Activities}

\begin{itemize}
\item	{\bf Technology Transfer:}
	Forged consulting relationships with several companies
	to aid industry deployment of several research results: e.g.,
	Mach microkernel code from the Flux project at Utah,
	NAT traversal for Voice over IP, and
	Persistent Personal Names system from the UIA project at MIT.

\item	{\bf Standards:}
	Regular participant in IETF (Internet Engineering Task Force)
	activities; in particular:
	\begin{itemize}
	\item	Co-author of two published RFCs (5128 and 5382)
		and several Internet-Drafts
	\item	Presented research in Transport Area meetings
		at IETF 70 (Dec 2007) and 73 (Nov 2008).
	\end{itemize}

\item	{\bf Service:}
	Program Committee member on ACM/CoNEXT ROADS 2008 workshop,
	ICCCN 2009 Peer-to-Peer Networking track, and OSDI 2010.

\item	{\bf Education:}
	As graduate student, co-developed educational JOS microkernel
	and associated curricula for MIT's operating system course.
\end{itemize}

\subsubsection*{(e) Collaborators \& Other Affiliations}

\begin{tabular}{ll}
\multicolumn{2}{c}{\bf Collaborators and Co-Editors} \\
Kaushik Biswas		& Cisco Systems, Inc. \\
Russ Cox		& Google, Inc. \\
Saikat Guha		& Cornell University \\
Janardhan Iyengar	& Franklin \& Marshall College \\
Chris Lesniewski-Laas	& Massachusetts Institute of Technology \\
Senthil Sivakumar	& Cisco Systems, Inc. \\
Pyda Srisuresh		& Kazeon Systems, Inc. \\
Jacob Strauss		& Massachusetts Institute of Technology \\
\\
\multicolumn{2}{c}{\bf Graduate Advisors and Postdoctoral Sponsors} \\
Frans Kaashoek		& Massachusetts Institute of Technology \\
Robert Morris		& Massachusetts Institute of Technology \\
Peter Druschel		& Max Planck Institute for Software Systems \\
\\
\multicolumn{2}{c}{\bf Thesis Advisor and Postgraduate-Scholar Sponsor} \\
Amittai Aviram		& Yale University \\
\end{tabular}



==> future.tex <==
\section{Future Directions}

file systems

dealing with general I/O - integrate with OS transactions?

Deterministic Transactional Memoryc:
allow intra-synchronization transactions to abort and rollback
if a conflict is detected at synchronization time,
deferring to one prioritized transaction among a conflicting set.

explore debugging dmachine processes -
good because nice and deterministic;
on the other hand, when a conflict occurs,
you might want some special support to trace back its cause.



==> math.tex <==
\subsection{Floating Point Determinism}

While most architecture features
are theoretically straightforward to canonicalize,
transcendental floating-point primitives
present a special problem due to their mathematical properties.
Floating-point operations inherently introduce round-off error,
and the only compelling way to standardize the results
of these operations precisely
is to require {\em exact rounding}:
for the implementation to behave
as if it had computed an infinitely-precise internal result
and then rounded that to yield the limited-precision answer.
{\em Algebraic} operations
such as $+$, $-$, $\times$, $\div$, and square root
can be exactly rounded efficiently~\cite{lang01bounds},
and common IEEE 754-compliant hardware already does so.

For non-algebraic operations
such as the exponential and trigonometric functions, however,
there is no known way to bound the precision required
of the function's internal result
in order to guarantee exact rounding,
other than by exhaustively exploring the floating-point operand space.
Such a search has been done for 32-bit operands~\cite{schulte94hardware},
and recently completed
for the 64-bit exponential functions~\cite{lefevre01worst};
64-bit trigonometric functions appear within reach~\cite{hanrot07worst}.
Exact rounding for the new 128-bit format
defined by IEEE 754-2008
will probably be out of reach for a while.
In any case, no current processors
guarantee exact rounding of non-algebraic functions
even when doing so is currently possible;
instead they just specify that the result is exactly rounded
with the possible exception of the least-significant bit,
whose error is implementation-defined
and hence potentially nondeterministic across different processors~\cite{
	intel09,amd07}.

\com{
Although there is no fundamental reason
the forms of architectural unpredictability discussed above
could not be fixed merely by changing the processor architecture
so as to specify all results precisely,
a basic mathematical problem currently presents a roadblock
against doing so for certain floating-point operations.
Floating-point operations must by definition compute
only approximations to their true real-number results,
rounded to some representable floating-point number.
In the interest of both computational precision and architectural determinism,
we would like {\em exact rounding},
where floating-point operations always yield
the closest representable floating-point number
to the operation's true mathematical real-number result
for the chosen rounding mode.
The problem is that real numbers theoretically have
an infinite number of digits,
and there is no {\em a priori} limit
on the number of significant digits one must compute
in order to produce an exactly rounded result of a given size.
For the special class of algebraic functions,
which include add, subtract, multiply, divide, and square root,
it is known how to bound the number of significant digits one must compute
in order to yield an exactly rounded result~\cite{lang01bounds},
and IEEE 754-compliant hardware already produces
exactly rounded (and hence deterministic) results
for these operations~\cite{XXX-ieee-754}.

For the non-algebraic transcendental functions
such as exponential, logarithmic, and trigonometric functions,
however,
no such analytical bound is available or likely to be forthcoming
without a mathematical breakthrough.
Determining the number of significant digits
an implementation must compute internally to produce an exactly-rounded result,
therefore,
essentially requires an exhaustive search
through the space of possible inputs
for a given floating-point precision.
Exactly rounded single-precision transcendental arithmetic
has been feasible for some time
due to the small 32-bit search space~\cite{schulte94hardware}.
Exactly rounded double-precision transcendentals
are much more challenging due to the 64-bit search space,
but recent advances have brought
exactly rounded exponential and logarithmic functions
into the realm of feasibility~\cite{lefevre01worst};
exact rounding for 64-bit trigonometric operations
is not yet possible but appears to be within reach~\cite{hanrot07worst}.
Exact rounding for the new 128-bit floating point format
defined by IEEE 754-2008~\cite{XXX}
is unlikely to be feasible any time soon.

Because of these difficulties,
instead of producing an exactly-rounded result,
current processors merely guarantee that the result computed
is correctly rounded with the possible exception
of the least significant bit~\cite{XXX-amd-and-intel-manuals}.
Under what conditions this least-significant digit is in error
depends on the internal details of the implementation,
the algorithms for which are generally proprietary
and thus not amenable to standardization across vendors.
Vendors are likely to resist guaranteeing exactly consistent results
even within a particular product line,
since by doing so they would give up freedom
to redesign internal algorithms for better performance or reduced cost.
}%com

\begin{figure}[t]
\centering
\includegraphics[width=0.45\textwidth]{../specbench/bench.eps}
\caption{Normalized SPEC floating-point benchmark results
	with native x87 floating-point operations enabled
	for all, exp/log only, or no transcendental math functions.}
\label{fig-fp}
\end{figure}

To provide full floating-point determinism on today's processors,
therefore,
our only option is to disable the problematic floating-point primitives
in the deterministic environment,
and require that applications use a software implementation instead.
A software implementation
will by definition always yield the same result
(even if inexactly rounded)
as long as the application is linked with the same math library.
The main concern then is
how seriously this emulation might impact performance.

\com{
Until exact rounding
at least for IEEE single- and double-precision floating-point
becomes feasible and supported by processors, therefore,
if we want a fully deterministic execution environment
our only choice is simply {\em not} to make
the problematic transcendental operations available
as primitives in the deterministic environment:
instead, application software running in the environment
must emulate these operations in software libraries.
Although such emulated implementations
may still yield inexactly-rounded results,
they will always yield {\em the same} inexact result on any execution
because the algorithm is contained within the deterministic environment.
The question, then, is the cost of this emulation.
}%com

As a preliminary experiment addressing this question,
we ran the SPEC CFP2006 floating-point benchmarks
linked against three variants of the GNU C library;
the results are shown in Figure~\ref{fig-fp},
normalized to the standard version of the C library (left bars).
The middle bars are for a C library
with exponential and logarithm operations in hardware
but trigonometric operations in software,
reflecting the fact that exact rounding is theoretically possible now
for the former operations but not the latter.
The right bars are for a C library
with all non-algebraic operations emulated,
as required to make current processors fully deterministic.
Most of the benchmarks see little impact,
but the {\tt bwaves} benchmark performs poorly
because of many exponentiations of the form $x^{3/4}$ in its inner loop.
Manually optimizing this operation into the mathematically equivalent
\verb|sqrt(sqrt(x*x*x))|
makes this performance impact disappear.
We therefore suspect that most applications, even if floating-point heavy,
would not greatly miss the hardware implementations
of these problematic operations.

\com{
To provide a preliminary answer to this question,
we ran the SPEC CFP2006 floating-point benchmarks on an x86 processor,
linking the benchmark against three variants of the GNU C library.
The first C library variant is unmodified,
and takes advantage of all the primitives the x87 FPU provides,
including all the non-algebraic operations subject to inexact rounding.
The second variant still uses the x87 FPU
to implement the transcendental and logarithmic functions---%
those for which exact rounding in single- and double-precision
is potentially feasible now,
although not yet supported by current processors---%
while the trigonometric operations use software implementations
that are included in the GNU C library but not usually used on x87 processors.
The third C library variant emulates
all non-algebraic transcendental operations in software.
Figure~\ref{fig-fp} shows the benchmark results,
normalized to the baseline C library variant.
Although all of these benchmarks make heavy use of floating-point arithmetic,
only three are noticeably impacted
by software emulation of the transcendental operations:
the rest depend primarily on the simple algebraic operations
for which current hardware already provides deterministic results.
Manual inspection reveals that the nearly 80\% slowdown of the bwaves benchmark
results from many ``inner-loop'' instances of raising a number
to the constant power $3/4$;
``manually optimizing'' this operation into the mathematically equivalent
\verb|sqrt(sqrt(x*x*x))|
makes the performance impact disappear.
Thus, we tentatively conclude that many floating-point applications
would be largely unaffected by the requirement
of emulating non-algebraic transcendentals in software
within a fully deterministic execution environment,
and that applications that are impacted
may still be able to run efficiently after minor modifications.
}%com


